Block4Forensic: An Integrated Lightweight Blockchain Framework for Forensics Applications of Connected Vehicles

Today's vehicles are becoming cyber-physical systems that do not only communicate with other vehicles but also gather various information from hundreds of sensors within them. These developments help create smart and connected (e.g., self-driving) vehicles that will introduce significant information to drivers, manufacturers, insurance companies and maintenance service providers for various applications. One such application that is becoming crucial with the introduction of self-driving cars is the forensic analysis for traffic accidents. The utilization of vehicle-related data can be instrumental in post-accident scenarios to find out the faulty party, particularly for self-driving vehicles. With the opportunity of being able to access various information on the cars, we propose a permissioned blockchain framework among the various elements involved to manage the collected vehicle-related data. Specifically, we first integrate Vehicular Public Key Management (VPKI) to the proposed blockchain to provide membership establishment and privacy. Next, we design a fragmented ledger that will store detailed data related to vehicle such as maintenance information/history, car diagnosis reports, etc. The proposed forensic framework enables trustless, traceable and privacy-aware post-accident analysis with minimal storage and processing overhead.

==> obsolete3_AccidentScene.tex <==
%\section{Preliminaries}
\subsection{Potential accident scene}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figs/Combined.pdf}
%\vspace{-0.3cm}
\caption{\small A Hypothetical accident scene and possible reconstructions of the accident. }\label{fig:scenario}
%\vspace{-0.3cm}
\end{figure*} 

An investigator working on an accident scene needs to collect all pieces of clues to reconstruct the accident scene. Once the accident scene is reconstructed, the faulty party can be determined accordingly. % Here, we discuss a possible accident scene and how the proposed B4F framework enable forensically sound accident scene reconstruction. 

% In a hypothetical case, Vehicle 1 and Vehicle 2 had a collision at an intersection with traffic lights. 
% -- we don't need to involve human angle, as this can even be automatized and handle machine2machine accidents. 
%Assume both sides deny liability and their testimonies about the case are not consistent.
%The accident and possible scenarios are shown in the center and around the center in Figure \ref{fig:scenario} respectively.

Here, we assume an accident scene where Vehicle 1 collided with Vehicle 2  at an intersection with traffic lights as illustrated in Fig.~\ref{fig:scenario}~(a). The data provided by B4F may enable various forensically sound scene reconstructions as listed below:
\begin{itemize}
\item \textbf{Reconstructed Scene (b)}: BSM messages include the traffic light status and  cars' last positions. In this scenario, BSM messages reveal that Vehicle 1 started to turn left when the red light was on as shown in Fig.~\ref{fig:scenario}~(b). Lights status data are being disseminated by the smart traffic lights and thus when the accident happens, B4F would have stored the last BSM messages from the traffic lights. Here, data clearly points out that the Vehicle 1 is the faulty party. 
%In this scenario, faulty party can easily determined by looking 

\item \textbf{Reconstructed Scene (c)}: Timestamped  data in B4F reveals the existence of another vehicle in the accident scene. Drivers of Vehicle 1 and Vehicle 2 started crossing the road when the light turned to green. At that time Vehicle 3 did not stop at red light and caused Vehicle 2 lost its control to hit Vehicle 1. B4F data uncovers the existence of Vehicle 3 and resolves such a hit case where faulty party is a third car that run out of the incident area.

\item \textbf{Reconstructed Scene (d)}: Similar to Scene (c), data reveals the existence of Vehicle 3. However, this time none of the cars violate the rules as the traffic light for Vehicle 3 is also green. BSM data supplied from smart traffic lights and other vehicles would reveal faulty signalization as the cause of the accident. 

\item \textbf{Reconstructed Scene (e)}: In this scenario B4F data indicates that none of the drivers violates the traffic rules. However, by investigating the car diagnostic report history on B4F, the investigator finds out that after maintenance, the vehicle has a left leaning problem while braking. Due to this faulty operation in Vehicle 1, the driver lost the control of the car and hit Vehicle 2. The history of previous vehicle maintenance records helps to resolve this complicated scenario and suggests maintenance provider as the faulty party. 

\item \textbf{Reconstructed Scene (f)}: In this scenario, B4F data shows that Vehicle 1 was on the autopilot at the accident time. Moreover, the diagnostic records report a failed sensor. Thus, Vehicle 1 autopilot software with faulty input caused the accident which suggests car manufacturer as the faulty party. 
%The investigator determine a malfunctioning component caused the accident by investigating previous history of car diagnostic reports.

\end{itemize}

Various parties might be involved in an accident like the example discussed above. Forensic data provided by B4F provides a fast and efficient accident scene reconstruction which will help any investigation significantly. Although a reconstruction might also be possible by traditional methods, it will not only be limited but also costly and time consuming. %its cost both in terms of time and money would be much higher. 


%https://www.lawinjury.com/press/blizzard-related-car-accident-case-settled-over-2-million

%https://www.mcdermotthickeylaw.com/vehicle-accident-case-stories/

%https://www.omicsonline.org/open-access/forensic-engineering-helps-in-accident-cases-analysis-a-review-2157-7145-1000390-94526.html

==> obsolete_4_VehicularForensicKeyFeatures.tex <==
\section{Key Features of Envisioned Forensic Analysis}
\label{sec:reqs}
The ultimate aim of vehicular forensics is to resolve disputes and determine the faulty parts in case of an accident. The developments in \emph{connected vehicles} provide new ways for forensic analysis by taking advantage of the IoT features discussed above. Different from the simplistic approach, utilizing produced sensors data with decision entities allows building a comprehensive vehicular forensic analysis. Considering involving multiple parties such as manufacturers, drivers, insurance companies, law enforcement etc., we identify the key features for an effective and trustworthy vehicular forensics as follows:


%\subsection{Key Features of envisioned vehicular forensic}

\begin{itemize}
\item{\textbf{Integrity:}} The integrity of forensic data is very important for resolving the disputes during forensic analysis.
\item{\textbf{Non-Repudiation:}} The parties should be held responsible for their actions by providing proof of the integrity and origin of data. 
\item{\textbf{Relieve Single Point-of-Trust:}} The system should remove trust solely to single authority and provide an accountable trustworthiness of each participant. 
\item{\textbf{Comprehensive Forensic Analysis:}} The system should provide a comprehensive mechanism to accident analysis via providing access to historical data even before the accident related data. For example, the behavioral pattern of vehicle after maintenance (i.e steering ability, braking distance) or a previously reported malfunctioning component of vehicle can give important clues to determine the faulty party.
\item{\textbf{Lightweightness:}} The system should have minimum overhead since it includes multiple parties that may have limited capabilities and resources.
\item{\textbf{Privacy:}} The system should preserve the privacy of the participants while also providing the flexibility for the participants to selectively reveal their data as they wish. However, the non-repudiation and integrity requirements should not be violated.
\end{itemize}


==> obsolete_RelatedWork.tex <==
%\section{Related Work}
%Usage of vehicle generated data in incident investigations has attracted the interest of the researchers. For instance, Nillson et. al.~\cite{nilsson2008conducting} discussed using the gathered information from vehicular networks (e.g. CAN bus, FlexRey and V2V communication) as forensic data. Another study analyzes Global Positing System (GPS) logs for enabling route reconstruction with the hope of resolving hit-and-run scenarios ~\cite{hoppe2012forensic}. Mansor et al.~\cite{mansor2016log} proposed to integrate vehicle with an authorized smartphone in order to collect data from the car for forensic investigations. Meanwhile, the ownership of EDR data and integrity of it is discussed in study ~\cite{kowalick500motor} along with how this data is used by Traffic Safety Administrator (NHTSA) and other third parties for post-accident scenario reconstruction.

%Authors in \cite{dorri2017blockchain} mention hypothetical usage of blockchain technology in information exchange for electric vehicles, however, their discussion lacks practical issues such as membership management, type and frequency of the data to be stored, data storage overhead and proof-of-work related computational overhead. 
%BlockChain: A Distributed Solution to Automotive Security and Privacy”, IEEE Communications Magazine, Volume 55, Issue 12, pages 119-125, December, 2017%Blockchain is currently being used in a broad range of areas with different Blockchain designs. 
%Since one of the major components in the proposed scheme is  data storage on Blockchain, rather than transferring assets using it ~\cite{nakamoto2008bitcoin}, we summarize the Blockchain design efforts for storing data. One related example is storing personal data of a user
%~\cite{chen2017personal,mainelli2016blockchain}. These studies create a digital identity of a user in Blockchain wallet validated once by an authority, and then used as an identity without sharing personal information when opening bank accounts, dealing with government institutes, etc. Another example is storing the ownership rights of assets \cite{de2016intellectual,bitcoin2015blockchain} to provide immutable ownership information and relieving the need of central authority with strong consensus. Blockchain usage is also suitable for tracking  product history on supply chain to identify counterfeit products and for facilitating origin of the product or storing data gathered from IoT devices (e.g., status of a shipment) with an immutable and accessible way \cite{vandon,hackius2017blockchain}. Storj and SiaCoin are other implementations utilizing Blockchain for monetizing the free disk space of the miners. However, they do not store data on the blockchain but the hashes of chunks of it, in order to satisfy integrity. Actual data storage takes place similar to ED2K  network.

%None of the existing schemes addresses the need for storing forensicly sound  data for connected vehicles with privacy guaranties. To the best of our knowledge, this is the first concrete framework providing a forensics layer for vehicle networks. 
